Security Analysis of Encrypted Virtual Machines

Cloud computing has become indispensable in today's computer landscape. The flexibility it offers for customers as well as for providers has become a crucial factor for large parts of the computer industry. Virtualization is the key technology that allows for sharing of hardware resources among different customers. The controlling software component, called hypervisor, provides a virtualized view of the computer resources and ensures separation of different guest virtual machines. However, this important cornerstone of cloud computing is not necessarily trustworthy. To mitigate this threat AMD introduced Secure Encrypted Virtualization, short SEV. SEV is a processor extension that encrypts guest memory in order to prevent a potentially malicious hypervisor from accessing guest data. In this paper we analyse whether the proposed features can resist a malicious hypervisor and discuss the trade-offs imposed by additional protection mechanisms. To do so, we developed a model of SEV's security capabilities based on the available documentation as actual silicon implementations are not yet on the market. We found that the currently proposed version of SEV is not up to the task owing to three design shortcomings. First, as with standard AMD-V, under SEV, the virtual machine control block is not encrypted and handled directly by the hypervisor, allowing him to bypass VM memory encryption by executing conveniently chosen gadgets. Secondly, the general purpose registers are not encrypted upon vmexit, leaking potentially sensitive data. Finally, the control of the nested pagetables allows a malicious hypervisor to closely control the execution of a VM and attack it with memory replay attacks.

==> as_design.tex <==
\subsubsection{Reversing the Guest Address Space}
\label{al}
The presented attack requires knowledge of the physical and/or the virtual load address of the guest kernel. 
Through the recent introduction of kernel space address randomization (KALSR), 
the kernel's sections are loaded at random virtual and physical offsets.
Here we present several ways to obtain the load address of the kernel text section inside the VM.
Given the load address all further function offsets can be obtained from the guest kernel binary statically.

\paragraph{Interrupt Injection}
The hypervisor can trigger the execution of certain functions (like interrupts) inside the guest.
By previously marking all guest memory pages as non executable through the nested pagetables, 
the guest will immediately fault revealing physical and virtual address of the function.
The physical address is revealed through the fault address stored in TODO: cr0?.
The virtual address can be obtained from the \textit{rip} register value stored in the \textit{vmcb}.
The load offset is then obtained by subtracting the leaked address from the function address obtained statically from the kernel binary.
Continuous guest execution is ensured, by resetting the guest state to values recorded before the interrupt injection.

\paragraph{Guest Control Registers}
The \textit{vmcb} exposes several control registers, pointing to kernel functions inside the guests virtual address space.
Again these virtual addresses can be compared against the reference address taken from the kernel binary to calculate the base load address.
Given the virtual address, the physical address can be obtained by causing a nested page fault through access of the virtual address.



==> ce_design.tex <==
\subsection{Arbitrary Code Execution}
\label{sec:ce}

